EPIC-Bench: A Perception-Centric Benchmark for Fine-Grained Embodied Visual Grounding in Vision-Language Models

While large vision-language models (VLMs) are increasingly adopted as the perceptual backbone for embodied agents, their fundamental vision-language grounding (VLG) capability in embodied scenarios remains unexplored. We present \textbf{EPIC-Bench}, \textbf{E}mbodied \textbf{P}ercept\textbf{I}on Ben\textbf{C}hmark, a fine-grained grounding benchmark designed to systematically evaluate the VLG capabilities of VLMs in real-world embodied environments. EPIC-Bench comprises 6.6k meticulously human-annotated tuples (Image, Text, Mask) spanning three core stages of the embodied interaction pipeline: Target Localization, Navigation, and Manipulation. With 23 fine-grained tasks, multi-dimensional settings and evaluation over 80 leading VLMs, EPIC-Bench provides a diagnostic analysis.

==> sections/abstract.tex <==

\begin{abstract}
While large vision-language models (VLMs) are increasingly adopted as the perceptual backbone for embodied agents, existing benchmarks often rely on question-answering or multiple-choice formats. These protocols allow models to exploit linguistic priors rather than demonstrating genuine visual grounding. To address this, we present \textbf{EPIC-Bench}, \textbf{E}mbodied \textbf{P}ercept\textbf{I}on Ben\textbf{C}hmark, a fine-grained grounding benchmark designed to systematically evaluate the visual perceptual capabilities of VLMs in real-world embodied environments. Comprising 6.6k meticulously annotated tuples (Image, Text, Mask), EPIC-Bench spans 23 fine-grained tasks across three core stages of the embodied interaction pipeline: Target Localization, Navigation, and Manipulation. 
Extensive evaluations of over 89 leading VLMs reveal that while advanced reasoning models show promise, current VLMs universally struggle with complex visual-text alignment for physical interactions. Specifically, models exhibit critical bottlenecks in multi-target counting, part-whole relationship understanding, and affordance region detection. EPIC-Bench provides a robust foundation and actionable insights for advancing the next generation of vision-driven embodied models.

%  First, it encourages genuine visually grounded perception without exploiting linguistic priors. Second, it comprises 23 fine-grained tasks spanning the embodied interaction pipeline from Target Localization to Navigation and Manipulation. Third, its fine-grained taxonomy supports diagnostic analysis of embodied visual perception.
% Comprehensive experiments show that VLMs still struggle to align visual–text information for downstream physical interactions, especially in affordance region detection, where the target is only part of an object.
% 或特别是当涉及到与可供性和接触关系有关的具身属性时。
% with Gemini 53.59 overall score, excel at 



% especially when there are multiple targets share the similar fine-grained attributes.



% Overall, EPIC-Bench provides a rigorous and comprehensive assessment of the visual perceptual competencies necessary for LVLMs to execute human instructions in embodied settings. Its fine-grained task taxonomy further offers actionable guidance for model selection in embodied agent construction and delineates critical directions for future training paradigms aimed at strengthening embodied intelligence.




% Embodied agents require fine-grained perceptual capabilities to ground language instructions into actionable representations. While recent advances in Vision-Language Models (VLMs) have significantly improved multimodal reasoning, existing benchmarks primarily emphasize coarse spatial reasoning and question answering, leaving critical embodied dimensions—such as target localization, navigation grounding, and manipulation-relevant perception—underexplored. As a result, current evaluation protocols may overestimate model competence in embodied settings.

% In this work, we introduce EPIC-Bench, a large-scale fine-grained grounding benchmark designed to evaluate the perceptual capabilities necessary for embodied intelligence. EPIC-Bench consists of three major categories, nine task types, and twenty-one subcategories, covering comprehensive embodied perception scenarios. To facilitate lightweight evaluation and rapid iteration, we further propose EPIC-Bench-Lite, a distilled core subset preserving the essential evaluation axes.

% We conduct extensive evaluations across a wide spectrum of state-of-the-art multimodal large models, spanning diverse model scales and architectures. Experimental results reveal that even the most advanced systems, including frontier proprietary and open-source models, exhibit substantial performance degradation under fine-grained grounding settings. Through detailed data and result analysis—including diversity, difficulty distribution, and annotation quality—we demonstrate that EPIC-Bench provides a more faithful assessment of embodied perceptual competence. We hope our benchmark can serve as a foundation for advancing fine-grained multimodal perception in embodied AI.
\end{abstract}


==> sections/evaluation.tex <==
\section{Evaluation Strategy}

\subsection{Evaluation Setup}
% To systematically assess embodied perception abilities, we evaluate 30+ leading VLMs on EPIC-Bench. We categorize VLMs into three categories: Proprietary Models, Open-Source Models, and Embodied Foundation Models. For proprietary models, inference is conducted via API calls, while the remaining two are deployed locally using the SWIFT framework. To eliminate randomness and ensure fairness, all experiments are conducted under identical settings, with final results reported as the average over multiple \textcolor{blue}{(how many?)} runs to reflect optimal performance. Detailed prompt designs for the different sub-task types in EPIC-Bench are provided in the Appendix.

To systematically assess embodied perception abilities, we evaluate 80+ leading VLMs on EPIC-Bench. These models are classified into three categories: Proprietary Models, Open-Source Models, and Embodied Foundation Models. 
% Inference for proprietary models is executed via API calls, whereas the latter two are deployed locally utilizing the ms-swift~\cite{zhao2024swiftascalablelightweightinfrastructure} framework. For proprietary models, inference is conducted via API calls, while the remaining two are deployed locally using the ms-swift~\cite{zhao2024swiftascalablelightweightinfrastructure} framework. 
To guarantee a fair comparison, all evaluations are conducted under identical settings. 
We report the average performance across 6 independent runs for locally deployed models. Given the empirically verified high stability and minimal variance across these runs, proprietary models are evaluated over 2 runs to maintain statistical reliability. Detailed prompt templates tailored to various sub-task types are provided in the Appendix.~\ref{app:prompts}.
% Open-source models are evaluated over 6 runs, showing highly stable results; proprietary models are thus evaluated over 2 runs with similar stability. Final results are reported as averages. Detailed prompt designs for the different sub-task types in EPIC-Bench are provided in the Appendix.







\subsection{Evaluation Metrics}

\begin{table*}[t!]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    % \fontsize{5}{5}\selectfont
    \renewcommand{\arraystretch}{1} % 统一行距
    \resizebox{\textwidth}{!}{%
    % \small
    \footnotesize
    \begin{tabular}{l@{} c@{\quad} lll lll lll}
    \toprule
    \multirow{3}{*}{\textbf{Model}}
        & \multirow{3}{*}{\textbf{Average}}
        & \multicolumn{3}{c}{\textbf{Target Local.}}
        & \multicolumn{3}{c}{\textbf{Navigation}}
        & \multicolumn{3}{c}{\textbf{Manipulation}} \\
    \cmidrule(r){3-5} \cmidrule(r){6-8} \cmidrule(r){9-11}
    &  & BA & SRA & ECA & GD & FP & VM & AR & CR & PR. \\
    \midrule

    \rowcolor{blue!8}[0pt][0pt]
    \multicolumn{11}{@{}c@{}}{\textbf{Proprietary Models}} \\
    Gemini-2.5-Pro$^{\dagger}$           & 37.63 & 42.86 & 41.62 & 36.43 & 9.630  & 46.29 & 42.70 & 8.720 & 33.94 & 42.78 \\
    Gemini-3-Pro$^{\dagger}$             & \cellcolor{green!10}\textbf{54.81} & \underline{56.81} & 54.50 & \cellcolor{green!10}\textbf{53.90} & \underline{48.82} & \cellcolor{green!10}\textbf{70.82} & \cellcolor{green!10}\textbf{60.08} & \cellcolor{green!10}\textbf{30.40} & \underline{51.78} & \underline{53.42} \\
    Gemini-3.1-Pro$^{\dagger}$           & \underline{54.72} & 55.38 & \cellcolor{green!10}\textbf{56.65} & \underline{53.04} & 47.22 & \underline{70.32} & \underline{59.06} & \underline{28.89} & \cellcolor{green!10}\textbf{53.70} & \cellcolor{green!10}\textbf{55.25} \\
    
    Claude-Sonnet-4.6$^{\dagger}$         & 43.24 & 45.43 & 45.49 & 36.47 & 40.16 & 68.46 & 42.77 & 9.790 & 46.21 & 43.81 \\
    
    o3$^{\dagger}$    & 36.05 & 39.37 & 40.96 & 32.86 & 36.24 & 30.64 & 40.73 & 5.49 & 32.43 & 43.64 \\
    GPT-5.4                                      & 38.95 & 43.78	&43.90	&33.84	&32.24	&43.12	&44.35	&8.670	&39.55	&37.30 \\
    GPT-5.5                                      & 50.16 & \textbf{57.78}	&\underline{55.37}	&45.19	&\textbf{50.97}	&38.57	&51.65	&24.62	&49.67	&48.70 \\
    
    Doubao-Seed-1.8$^{\dagger}$           & 46.32 & 55.29 & 49.68  & 46.10 & 46.02 & 53.43 & 45.90 & 10.94 & 14.36 & 40.79 \\
    Doubao-Seed-1.6-Vision$^{\dagger}$    & 46.80 & 54.64 & 49.92  & 42.27 & 41.64 & 58.74 & 42.66 & 9.520 & 47.48 & 41.62 \\

    Qwen3.6-Plus$^{\dagger}$              & 45.48 & 47.66 & 50.17  & 41.07 & 44.47 & 62.12 & 41.57 & 11.95 & 47.84 & 41.59 \\
    Qwen3.5-Plus$^{\dagger}$              & 47.10 & 55.09 & 51.90  & 41.82 & 50.85 & 57.89 & 45.21 & 13.82 & 22.34 & 42.46 \\
    Qwen3.6-35B-A3B$^{\dagger}$           & 35.07 & 48.17 & 43.99  & 36.61 & 14.41 & 33.97 & 21.30 & 2.840 & 17.05 & 15.90 \\

    HunYuan-T1-Vision$^{\dagger}$         & 43.00 & 51.24 & 47.60  & 39.67 & 42.63 & 50.08 & 33.54 & 6.630  & 38.95 & 34.49 \\
    HunYuan-Vision-1.5                    & 32.55 & 38.37 & 39.60 & 29.67 & 31.72 & 17.07 & 35.71  & 6.380  & 32.88 & 29.25 \\

    
    \midrule
    
    \rowcolor{blue!8}[0pt][0pt]
    \multicolumn{11}{@{}c@{}}{\textbf{Open-source Models}} \\
    Qwen3.6-35B-A3B                     & 38.52 & 46.40 & 46.19 & 40.01 &  3.900 & 39.16 & 39.42 &  5.410 & 34.19 & 34.52 \\

    Qwen3.5-397B-A17B$^{\dagger}$       & \underline{47.47} & \underline{55.45} & 51.82 & 42.10  & 51.10  & \underline{60.11} & \underline{45.35} & 12.40  & 26.33 & \underline{42.51} \\
    Qwen3.5-397B-A17B                   & 45.16 & 50.56 & 50.06 & \underline{43.45} & \cellcolor{green!10}\textbf{51.94} & 50.61 & 41.46 & 8.310  & 34.51 & 37.08 \\
    Qwen3.5-122B-A10B$^{\dagger}$       & 47.24 & 53.61 & 49.13 & 41.16 & \underline{51.42} & \textbf{63.47} & 45.19 & 12.31 & \underline{46.04} & 39.77 \\
    Qwen3.5-122B-A10B                   & 44.54 & 50.77 & 49.28 & 42.31 & 49.65 & 50.50  & 42.62 & 8.300  & 36.91 & 32.16 \\

    Qwen3-VL-235B-A22B$^{\dagger}$      & \textbf{50.93} & \cellcolor{green!10}\textbf{58.00} & \textbf{55.67} & \textbf{48.12} & 48.18 & 51.19 & \textbf{49.01} & \underline{16.96} & \textbf{48.04} & \textbf{46.49} \\
    Qwen3-VL-235B-A22B  & 42.64 & 50.12 & 45.86 & 39.34 & 50.96 & 43.14 & 38.69 & 12.00 & 34.55 & 35.71 \\
    
    Qwen2.5-VL-72B & 42.51 & 47.54 & 49.79 & 40.92 & 49.45 & 42.49 & 37.08 & 14.77 & 21.21 & 35.90 \\

    InternVL3.5-241B-A28B & 40.75 & 44.65 & 50.59 & 37.61 & 35.94 & 35.47 & 33.73 & 16.85 & 36.41 & 37.60 \\
    InternVL3.5-38B                               & 42.54 & 48.69 & \underline{52.60} & 39.95 & 43.21 & 35.01 & 28.07 & \textbf{17.22} & 34.05 & 35.83 \\
    InternVL3.5-30B-A3B                           & 29.71 & 30.96 & 39.11 & 27.03 & 45.43 & 24.11 & 17.24 & 8.410  & 18.75 & 25.30 \\

    InternVL3-78B                                 & 36.04 & 40.68 & 44.56 & 32.78 & 35.98 & 30.55 & 34.93 & 6.900  & 29.07 & 31.69 \\

    MiMo-VL-7B-RL-2508                            &34.65	&36.65&	42.31	&34.92	&18.31	&36.90	&37.45	&6.510	&30.37&	32.86 \\
    Gemma-3-27B-IT                                & 27.17 & 26.93 & 33.66 & 26.68 & 11.62 & 32.17 & 26.33 & 1.650  & 31.26 & 32.18 \\
    GLM-4.6V$^{\dagger}$                          & 42.84 & 50.19 & 47.71 & 37.89 & 42.46 & 51.11 & 36.55 & 8.320  & 34.14 & 39.79 \\
    Step3-VL-10B                                  & 32.40 & 42.22 & 40.10 & 31.88 & 17.96 & 24.03 & 17.77 & 5.940  & 27.22 & 27.56 \\
    LLaVA-NeXT-72B                                & 20.40 & 26.54 & 29.42 & 19.93 & 14.18 & 6.340  & 6.190  & 2.990  & 12.75 & 18.63 \\
    \midrule

    \rowcolor{blue!8}[0pt][0pt]
    \multicolumn{11}{@{}c@{}}{\textbf{Embodied Foundation Models}} \\
    Pelican1.0-VL-72B                             & \underline{35.29} & \underline{44.08} & \underline{42.11} & \underline{34.79} & \textbf{44.91} & 0.000  & \textbf{38.13} & \textbf{7.320} & 22.68 & \underline{37.96} \\

    RoboBrain2-32B                                & \textbf{39.32} & \textbf{50.66} & \textbf{49.67} & \textbf{38.83} & \underline{38.85} & 0.610  & \underline{37.63} & 0.080 & \textbf{36.22} & \textbf{39.61} \\
    
    RoboBrain2.5-8B-NV                            & 23.81 & 24.81 & 32.88 & 24.97 & 22.57 & 1.660  & 27.98 & 1.130 & 24.98 & 24.03 \\
    RoboBrain2.5-8B-MT                            & 29.83 & 31.20 & 37.41 & 26.76 & 33.52 & \textbf{30.89} & 27.84 & 2.650 & \underline{25.45} & 24.34 \\
    
    RynnBrain-8B                                  & 22.34 & 28.31 & 33.28 & 24.81 & 7.980  & 5.950  & 15.04 & 0.130 & 13.84 & 11.26 \\
    RynnBrain-CoP-8B                              & 16.83 & 12.48 & 21.78 & 16.08 & 21.51 & \underline{22.51} & 13.58 & 0.280 & 19.62 & 18.09 \\
    RynnBrain-Plan-8B                             & 23.59 & 23.53 & 32.53 & 26.08 & 2.120 & 19.57  & 21.41 & 0.110 & 18.79 & 31.02 \\
    
    VeBrain                                       & 29.27 &	33.63 &	35.98 & 27.69 & 29.56 &	20.04  & 27.58 & 2.850&19.25 & 32.30 \\
    Cosmos-Reason1-7B                             & 23.25 & 29.74 & 26.64 & 19.67 & 24.68 & 3.030  & 25.44 & \underline{5.370} & 22.12 & 32.75 \\

    \bottomrule
    \end{tabular}
    }
    \caption{
        Overall performance of representative VLMs on EPIC-Bench.
        \colorbox{green!10}{\textbf{Green bold}} indicates the overall best result across all models.
        \textbf{Bold} and \underline{underline} indicate the best and second-best results within each model category, respectively.
        $^{\dagger}$ denotes models evaluated with thinking mode enabled.
        Comprehensive results for all evaluated models are provided in Tab.~\ref{tab:table-performance-full} of Appendix.~\ref{app:additional_results}.
    }
    \label{tab:table-performance-select}
\end{table*}


Our evaluation framework employs task-specific metrics. As detailed in Tab.~\ref{tab:Score_Composition}, the overall scoring system comprises four components: Localization Score, Counting Score, Path Score, and a binary Feasibility Score. Each task selects an appropriate subset of these metrics according to its characteristics. For an individual sample in a specific task, the final score is the weighted average of its selected metrics. The benchmark's overall score is then computed as the average across all data samples. We detail the scoring criteria for each metric below.


\paragraph{Localization Score.} This metric evaluates the model's ability to precisely ground target objects. Acknowledging the output format limitations of current VLMs, we prompt models to predict bounding boxes (Bboxes) indicating target locations. To compute the IoU against our fine-grained ground-truth (GT) masks, the predicted Bbox is instantiated as a solid rectangular mask. This rectangular approximation is then directly compared with the GT mask to calculate the final localization score.

\paragraph{Counting Score.} This score measures the model's vision-language alignment ability by requiring it to predict the exact number of valid targets matching the textual description. The scoring function adapts based on a binary \textit{precise count} label in the ground truth. If the precise count is strictly required (True), we apply a binary accuracy:

\begin{equation}
\text{Count\_Score} = \begin{cases} 1 & \text{if } \text{Predict\_Count} = \text{GT\_Count} \\ 0 & \text{otherwise} \end{cases}
\end{equation}

If the precise count is not strictly required (False), we apply a soft penalty for numerical deviations:
\begin{equation}
\max\left(1 - \frac{|\text{Predict\_Count} - \text{GT\_Count}|}{\text{GT\_Count}},\ 0\right) \nonumber
\end{equation}


% \begin{table*}[t!]
% \centering
% \resizebox{\textwidth}{!}{
%     % \setlength{\tabcolsep}{8pt}
%     \fontsize{7}{7}\selectfont
%     \begin{tabularx}{\textwidth}{l|l}
%     \toprule
%      Task Type & Score Composition \\
%     \midrule
%     TL-All & $(1-\alpha)$ Localization Score + $\alpha$  Counting Score \\
%     \midrule
%     NAV-Ground Detection & Localization Score \\
%     NAV-Feasible Path & Path Score \\
%     NAV-Visual Matching & $(1-\alpha)$ Localization Score + $\alpha$ Counting Score \\
%     \midrule
%     MAN-Affordance Region & Localization Score \\
%     MAN-Contact Relationship & $(1-\alpha)$ Localization Score + $\alpha$  Counting Score \\
%     MAN-Placement Region & $(1-\alpha)$ Localization Score + $\alpha$  Feasibility Score \\
%     \bottomrule
%     \end{tabularx}
%     }
%     \caption{Task-specific score compositions. The weighting factor $\alpha$ defaults to 0.5. Exceptions: (1) For TL, $\alpha = 0.3$ if the GT precise count label is False or if the textual instruction contains explicit numerical information. (2) For MAN-CR, $\alpha = 0.3$ if the GT precise count label is False.} \label{tab:Score_Composition}
% \end{table*}

\begin{table}[t]
\centering
\small
\resizebox{8cm}{!}{
\begin{tabular}{l l}
\toprule
\textbf{Task Type} & \textbf{Score Composition} \\
\midrule
TL-All &
$(1-\alpha)\,\text{Localization Score} + \alpha\,\text{Counting Score}$ \\
\midrule
NAV-Ground Detection &
Localization Score \\
NAV-Feasible Path &
Path Score \\
NAV-Visual Matching &
$(1-\alpha)\,\text{Localization Score} + \alpha\,\text{Counting Score}$ \\
\midrule
MAN-Affordance Region &
Localization Score \\
MAN-Contact Relationship &
$(1-\alpha)\,\text{Localization Score} + \alpha\,\text{Counting Score}$ \\
MAN-Placement Region &
$(1-\alpha)\,\text{Localization Score} + \alpha\,\text{Feasibility Score}$ \\
\bottomrule
\end{tabular}
}
\caption{Task-specific score compositions. The weighting factor $\alpha$ defaults to 0.5. Exceptions: (1) For TL, $\alpha = 0.3$ if the GT precise count label is False or $\alpha = 0.1$ if the textual instruction contains explicit numerical information. (2) For MAN-CR, $\alpha = 0.3$ if the GT precise count label is False.} \label{tab:Score_Composition}
\end{table}


\paragraph{Path Score.} This metric assesses the model's capacity to plan a valid, traversable route. It aggregates five sub-components: start/end point accuracy, path reasonableness, distance from the start, proximity to the destination, and path continuity. Models are required to output at least three consecutive point coordinates representing the trajectory, constrained within navigable ground regions. Detailed scoring formulations are provided in the Appendix.~\ref{app:path_score}.


\paragraph{Feasibility Score.} The feasibility score evaluates the model's physical common sense regarding task execution in a binary format. For example, in the placement region assessment task, the model must determine whether a proposed placement action is physically viable, requiring joint reasoning over the size, geometry, and stability of both the manipulated object and the target receptacle.






% \subsection{ANALYSIS}

% % 整体三大类分数情况
% \subsubsection{ Overall Analysis }
%    As shown in \Cref{fig:Overall}. The overall score of three major task categories.  TL>NVG>MANP,specifically:
% \begin{itemize}
%     \item 1)In TL, BasicAttributes close to SpatialRelatedAtributes, EmbodiedCompositionnalAttributes Worst.
%     \item 2)In NVG, all close, but for Internvl3.5-241B and Qwen3-235-instruct, GD>FP>VM.
%     \item 3)In MANP, AffordanceRegion largely fall behind.
% \end{itemize}


% % \begin{figure}[tb]
% %   \centering
% %   \includegraphics[height=4.5cm]{Graphics/Analysis/Overall/Qwen3-VL/Qwen3-VL-235B-A22B-Thinking/Qwen3-VL-235B-A22B-Thinking-combined.png}
% %   \caption{ The overall score of three major task categories.  TL>NVG>MANP，Specifically,1)In TL, BasicAttributes close to SpatialRelatedAtributes, EmbodiedCompositionnalAttributes Worst.   2)In NVG, all close, but for Internvl3.5-241B and Qwen3-235-instruct, GD>FP>VM. 3)In MANP, AffordanceRegion largely fall behind.}
% %   \label{fig:Overall}
% % \end{figure}

% % 目标定位大类结果分析，包括1）该大类下各子类的得分分析（暂时只看绿色部分） +2）计数得分与是否精确计数的关系，
% \subsubsection{ TargerLocalization Analysis }


% % 子类得分分析
%  1) \textbf{Subtask scores} As shown in \Cref{fig:TL_subtask},
%  the detail scores of subtask of TL, Embodied related Attributes get the lowest average score,
%   but Color,Geometry,PartWhole , Spoken , Orientation related subtask worst, cuz these types of attributes/taskset are rare to seen in General Training dataset, but these subtask are important

% % \begin{figure}[tb]
% %   \centering
% %   \includegraphics[height=4.5cm]{Graphics/Analysis/Overall/Qwen3-VL/Qwen3-VL-235B-A22B-Thinking/Qwen3-VL-235B-A22B-Thinking-by-subtask.png}
% %   \caption{ The detail score of subtask of TL, Embodied related Attributes get the lowest avrage score,
% %   but Color,Geometry,PartWhole ,Spoken , Orientation_related subtask worst, cuz these types of attributes/task_set are rare to seen in General Training dataset, but these subtask are important
% %   }
% %   \label{fig:TL_subtask}
% % \end{figure}



% % 计数得分分析,包括1）GT标签为精确计数时，计数得分分析+2）标签中已经包含数量时，计数得分分析
% 2)\textbf{Count Score}
% \begin{itemize}
% % 1）GT标签为精确计数时，计数得分分析

%     \item \textbf{Precise Count Group}As shown in \Cref{fig:TL_CountScore_Precise_Count},The score distribution according to the number of target instance, where \textbf{Precise Count is true} the y-axis equivalent to the acc , as the number of target increase(>1),the acc drops,, which suggest  1) current LMMs fail to match the visual-text info when there are multiple targets satisfy the requirement.
%   2) the shortage of Target Localization ability or visual-text alignment ability revealed by our benchmark, is not the side affect of poor grounding ability. LMMs cannot even get the number right

% % \begin{figure}[tb]
% %   \centering
% %   \includegraphics[height=4.5cm]{Graphics/Analysis/TL_CountScore_by_Weight/Qwen3-VL/Qwen3-VL-235B-A22B-Thinking/Qwen3-VL-235B-A22B-Thinking-tl-count-score-wc0_5.png}
% %   \caption{ The score distribution according to the number of target instance, where \textbf{Precise Count is true}. the y-axis equivalent to the acc , as the number of target increase(>1),the acc drops,, which suggest  1) current LMMs fail to match the visual-text info when there are multiple targets satisfy the requirement.
% %   2) the shortage of Target Localization ability or visual-text alignment ability revealed by our benchmark, is not the side affect of poor grounding ability. LMMs cannot even get the count task right
  
% %   }
% %   \label{fig:TL_CountScore_Precise_Count}
% % \end{figure}
% % \end{itemize}




% % 2）标签中已经包含数量时，计数得分分析（QWen3vl-235b没有问题，但是Internvl3.5241B比较差，晚点替换成多个模型的结果对比图）
% \begin{itemize}
%     \item \textbf{With number in label Group} As shown in \Cref{fig:TL_CountScore_Number_in_Label}, The score distribution according to the number of target instance, where \textbf{The number of targets is already shown in Grounding Text Label}. the y-axis equivalent overall acc, this suggest some LMMs fails to effectively get numeric info from text info.



% % \begin{figure}[tb]
% %   \centering
% %   \includegraphics[height=4.5cm]{Graphics/Analysis/TL_CountScore_by_Weight/InternVL3.5/InternVL3.5-241B-A28B/InternVL3.5-241B-A28B-tl-count-score-wc0_1.png}
% %   \caption{ The score distribution according to the number of target instance, where \textbf{The number of targets is already shown in Grounding Text Label}. the y-axis equivalent overall acc, this suggest some LMMs fails to effectively get numeric info from text info.
  
% %   }
% %   \label{fig:TL_CountScore_Number_in_Label}
% % \end{figure}

% % \end{itemize}



% % 导航与操作大类结果分析，包括1）overlay作为视觉提示的作用（验证输入时 是否提供被操作目标overlay 对  得分 的影响，   ）+2）Case Study ，模型倾向于标记出操作目标整体，而不是具体的可供性区域，与“TL大类中部分与整体子类得分低相关程度很大（属于推测，暂时没有实验数据验证）”
% \subsubsection{ NVG and MANI  Analysis }



% % 导航大类结果分析，
% 1) \textbf{Navigation Analysis}


% % 需不需要考虑使用 EPIC-Bench 进行监督微调，然后在另外一个benchmark上进行测评，以验证 EPIC-Bench 覆盖的维度的可以提高模型相关维度的能力



==> sections/exp.tex <==


\section{Experiments}

In this section, we present the evaluation and ablation results of representative mainstream models. Section \ref{sec:overall} reports the overall performance, Section \ref{sec:TL} analyzes Target Localization capabilities, Section \ref{sec:NAV_MAN} evaluates Navigation and Manipulation perception tasks, and Section \ref{sec:model_efficiency} examines model efficiency across different scales and modes.

% \begin{figure*}[t!]
%   \centering
%   \includegraphics[width=\textwidth]{Graphics/combined_radar_round_001.pdf}
%   \caption{Representative VLM performance on 23 tasks of Epic-Bench.}
%   \label{fig:5.2.1_5.3.1}
% \end{figure*}

\subsection{Overall Model Performance} \label{sec:overall}
Tab.~\ref{tab:table-performance-select} summarizes the overall performance of representative VLMs on EPIC-Bench, with comprehensive results provided in the Appendix.~\ref{app:additional_results}. We derive three key observations. First, Among proprietary models, Gemini-3-Pro and Gemini-3.1-Pro achieve the strongest overall performance, with average scores above 54.77. Among open-source models, Qwen3-VL-235B-A22B-thinking obtains the best overall result, while both models struggle with the AR task, Gemini-3-Pro-Thinking achieves the highest score (70.82) on the FP task. Second, the top-performing models are predominantly ``thinking'' variants. Under comparable architectures and parameter scales, models equipped with advanced reasoning modes consistently outperform their standard counterparts. Third, current embodied foundation models do not exhibit particularly strong performance on our benchmark; this can primarily be attributed to their relatively smaller parameter scales.

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\textwidth]{Graphics/num_score_0305.pdf}
  \caption{Counting accuracy across different numbers of target objects on ContactRelationship and TargetLocalization tasks.}
  \label{fig:number_score}
\end{figure*}

\subsection{Analysis of Target Localization} \label{sec:TL}
In this section, we first identify weaknesses in the vision–language alignment of current models. We then conduct controlled experiments to disentangle localization from alignment abilities, highlighting the perceptual reasoning gap between models and human baselines.

\paragraph{Fine-Grained Result Analysis.}
% Target Localization is divided into 14 sub-tasks to precisely diagnose deficiencies across different dimensions of vision–language alignment. 
Fig.~\ref{fig:5.2.1_5.3.1}(a) reports the fine-grained performance across TL sub-tasks.
First, models struggle significantly with Part-Whole relationships. While capable of holistic object localization, they fail to ground specific sub-regions based on textual descriptions. This deficiency directly contributes to their poor performance on Affordance Region tasks (detailed in Section~\ref{sec:NAV_MAN}).
Second, models exhibit a strong bias toward localizing only the most salient instance, whereas our benchmark requires exhaustive grounding of all valid targets. This bias leads to sub-optimal results on conventional basic-attribute tasks, particularly color and material recognition. 
Finally, performance degrades substantially on spatial orientation tasks, highlighting a lack of robust spatial reasoning and reference-frame comprehension in current VLMs.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{Graphics/Round_002_combined_radar.pdf}
  \caption{Representative VLM performance on 23 tasks of Epic-Bench.}
  \label{fig:5.2.1_5.3.1}
\end{figure*}

\paragraph{Decoupled Analysis of Localization and Vision-Language Alignment.} Our evaluation requires models to predict both the target count and the corresponding Bbox. This raises a critical question: do low scores stem from poor vision–language alignment or inaccurate box prediction?
To investigate, we select samples from the TL and MAN-CR tasks where the precise label is strictly required. We compare counting accuracy under two settings: (1) joint localization-and-counting, and (2) counting-only, predicting the count without bounding boxes.
As shown in Tab.~\ref{tab:fig_5.2.2}, counting performance remains largely consistent across settings. Surprisingly, the joint condition slightly outperforms the counting-only setting. We hypothesize that the explicit requirement of box prediction encourages more deliberate reasoning over visual regions, prompting deeper visual engagement.

% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=\textwidth]{Graphics/single_big.pdf}
%   \caption{Performance comparison under joint localization–counting and counting-only evaluation settings on TL and MAN-CR tasks with precise-count annotations.}
%   \label{fig:5.2.2}
% \end{figure}

% \begin{table}[t]
%   \centering
%   \caption{}
%   \label{tab:overlay_comparison}

%   \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l| c c| c c c}
%       \toprule
%       Overlay Type & 
%       Claude-Sonnet-4-6-Thinking & 
%       \makecell{Qwen3-VL-235B-\\A22B-Thinking} & 
%       \makecell{Qwen3.5-\\122B-A10B} & 
%       \makecell{Qwen3-VL-235B-\\A22B-Instruct} & 
%       \makecell{InternVL-3.5-\\241B-A28B} \\
%       \midrule
%       Mask(Base)    & 45.38 & 41.73 & 43.12 & 32.7 & 32.28 \\
%       Bbox          & 36.77 (-9.89\%)& 37.6(-9.89\%)  & 43.97(+1.97\%) & 32.85(+4.58\%) & 32.79(+1.57\%) \\
%       W/o Overlay   & 33.95(-14.78\%) & 35.56(-14.78\%)  & 41.18(-4.49\%)& 28.9(-11.62\%) & 31.61(-2.08\%) \\
%       \bottomrule
%     \end{tabular}
%   }
% \end{table}

% \begin{table}[t]
%   \centering
%   \caption{Performance comparison between Thinking and Instruct models under different overlay types.}
%   \label{tab:overlay_comparison}
%   \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l| c c| c c| c c| c c| c c| c c}
%       \toprule
%       & \multicolumn{2}{c|}{Qwen3-VL-235B-A22B} & \multicolumn{2}{c|}{Qwen3-VL-32B} & \multicolumn{2}{c|}{Qwen3-VL-30B-A3B} & \multicolumn{2}{c|}{Qwen3-VL-8B} & \multicolumn{2}{c|}{Qwen3-VL-4B} & \multicolumn{2}{c}{Qwen3-VL-2B} \\
%       \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
%       Max new token & Think & Inst & Think & Inst & Think & Inst & Think & Inst & Think & Inst & Think & Inst \\
%       \midrule
%       4096          &  &  &  &  &  &  &  &  &  &  &  &  \\
%       8192   &  &  &  &  &  &  &  &  &  &  &  &  \\
%       \bottomrule
%     \end{tabular}
%   }
% \end{table}


% \end{table}
% \begin{table}[t]
%   \centering
%   \caption{Performance comparison between Thinking and Instruct models under different overlay types.}
%   \label{tab:overlay_comparison}
%   \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l| c c| c c}
%       \toprule
%       & \multicolumn{2}{c|}{Thinking} & \multicolumn{2}{c}{Instruct} \\
%       \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%       \multirow{-2}{*}{\hspace{3em}Model} & 4096 & 8192 & 4096 & 8192 \\
%       \midrule
%       Qwen3-VL-235B-A22B & 40.99 & 50.93 & 37.28 & 42.64 \\
%       Qwen3-VL-32B       & 32.7  & 37.08 & 34.99 & 35.21 \\
%       Qwen3-VL-30B-A3B   & 41    & 44.02 & 30.44 & 30.60 \\
%       Qwen3-VL-8B        & 24.22 & 34.2  & 33.82 & 34.14 \\
%       Qwen3-VL-4B        & 23.77 & 32.47 & 33.32 & 33.05 \\
%       Qwen3-VL-2B        & 20.43 & 28.84 & 32.36 & 32.54 \\
%       \bottomrule
%     \end{tabular}
%   }
% \end{table}

% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=\textwidth]{Thinking-Instruct-Compare.pdf}
%   \caption{Performance comparison between Thinking and Instruct models under different overlay types. Visual prompts yield gains for all models, with Thinking models better leveraging masks and Instruct models favoring the familiar bbox format.}
%   \label{fig:overlay_ablation}
% \end{figure}


\paragraph{Relationship Between Counting Accuracy and Target Quantity.}
Why does counting accuracy remain unsatisfactory? To better understand this issue, we analyze the relationship between counting accuracy and the number of target objects in Fig.~\ref{fig:number_score}, models achieve near-human performance when exactly one target is present. However, accuracy degrades substantially in zero-target or multi-target scenarios. We attribute this trend to biases in vision-language alignment training data. Many widely used datasets, such as RefCOCO, predominantly assume a single target per image. Consequently, models are prone to hallucinating detections in zero-target scenarios or failing to identify all valid instances in multi-target settings.




\subsection{Analysis of Navigation and Manipulation} \label{sec:NAV_MAN}

In this section, we evaluate model performance on perception tasks critical for navigation and manipulation. Furthermore, we design ablation studies to assess the effectiveness of overlay-based visual prompts in assisting VLMs with these downstream tasks.

\paragraph{Fine-Grained Result Analysis.} As depicted in Fig.~\ref{fig:5.2.1_5.3.1}(b), VLMs achieve only moderate performance on navigation and manipulation tasks, with Affordance Region recognition yielding the lowest accuracy. As shown in Fig.~\ref{fig:5.3.1_case}, these two types of tasks are highly correlated and are crucial for downstream embodied applications. However, even leading models struggle to precisely localize target regions that correspond to specific parts of an object.

% \begin{figure}[tb]
%   \centering
%   \includegraphics[height=4.5cm]{Graphics/chapter_5/5.3.1.png}
%   \caption{xxxx}
%   \label{fig:5.3.1}
% \end{figure}

\begin{figure*}[tb]
  \centering
  \includegraphics[width=0.95\textwidth]{Graphics/chapter_5/5.3.1_case.png}
  \caption{Case study of Part-Whole and Affordance Region Tasks.}
  \label{fig:5.3.1_case}
\end{figure*}

\begin{figure}[tb]
  \centering
  \begin{subfigure}{0.46\textwidth}
  \includegraphics[width=\linewidth]{Graphics/5.4bar_chart.pdf}
    \caption{Impact of max new token length on model performance.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.46\textwidth}
  \includegraphics[width=\linewidth]{Graphics/tradeoff.pdf}
    \caption{Performance-Efficiency trade-off.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Efficiency assessment of Qwen3-VL model family.}
  \label{fig:short}
\end{figure}


\paragraph{Effect of Overlay as Visual Prompt.} To isolate reasoning capabilities from pure localization difficulty in complex navigation and manipulation tasks (i.e., Feasible Path, Affordance Region, Contact Relationship, and Placement Region), we evaluate three input settings: \textit{mask overlay}, \textit{Bbox overlay}, and \textit{no-overlay}. 
As shown in Tab.~\ref{tab:overlay_bbox_mask_comparison}, the no-overlay baseline consistently yields the lowest accuracy. While introducing visual prompts universally improves performance, the optimal format depends on the model's inherent capacity. Specifically, models with advanced reasoning capabilities effectively exploit the dense contextual geometry provided by \textit{mask overlays}, yielding the most substantial performance gains. Conversely, less capable models struggle to parse this rich visual information, often treating it as distracting noise. Instead, these models benefit more from the addition of simpler \textit{Bbox overlays}, which closely align with the familiar input formats encountered during their standard training paradigms.


% \begin{figure}[tb]
%   \centering
%   \includegraphics[height=4.5cm]{Graphics/chapter_5/5.3.2.png}
%   \caption{xxxx}
%   \label{fig:5.3.2}
% \end{figure}



% \textbf{Effect of IoU Threshold on Pass Rate.} In the current evaluation, IoU is used directly as the localization score. We therefore compare the effect of varying IoU thresholds on pass rates. As shown in Figure~\ref{fig:5.3.3} .

% \begin{figure}[tb]
%   \centering
%   \includegraphics[height=4.5cm]{Graphics/iou_passrate_round_001.pdf}
%   \caption{Pass rate over IoU Threshold.}
%   \label{fig:5.3.3}
% \end{figure}



% \begin{figure}[tb]
%   \centering
%   \begin{subfigure}{0.49\textwidth}
%   \includegraphics[width=\linewidth]{Graphics/tradeoff.pdf}
%     \caption{Performance-Efficiency trade-off.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.49\textwidth}
%   \includegraphics[width=\linewidth]{Graphics/5.4bar_chart.pdf}
%     \caption{Impact of max new token length on model performance.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Efficiency assessment of Qwen3-VL model family.}
%   \label{fig:short}
% \end{figure}
% \begin{figure}[tb]
%   \centering
%   \begin{subfigure}{0.49\textwidth}
%     \includegraphics[width=\linewidth]{Graphics/tradeoff.pdf}
%     \caption{Performance–efficiency trade-off of Qwen3-VL models.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.49\textwidth}
%     \centering
%     \resizebox{\linewidth}{!}{%
%       \begin{tabular}{l| c c| c c}
%         \toprule
%         & \multicolumn{2}{c|}{Thinking} & \multicolumn{2}{c}{Instruct} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%         \multirow{-2}{*}{Model} & 4096 & 8192 & 4096 & 8192 \\
%         \midrule
%         Qwen3-VL-235B-A22B & 40.99 & 50.93 & 37.28 & 42.64 \\
%         Qwen3-VL-32B       & 32.7  & 37.08 & 34.99 & 35.21 \\
%         Qwen3-VL-30B-A3B   & 41    & 44.02 & 30.44 & 30.60 \\
%         Qwen3-VL-8B        & 24.22 & 34.2  & 33.82 & 34.14 \\
%         Qwen3-VL-4B        & 23.77 & 32.47 & 33.32 & 33.05 \\
%         Qwen3-VL-2B        & 20.43 & 28.84 & 32.36 & 32.54 \\
%         \bottomrule
%       \end{tabular}
%     }
%     \caption{Impact of max new token length on model performance.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Efficiency of Qwen3-VL model family.}
%   \label{fig:short}
% \end{figure}



% \begin{figure}[tb]
%   \centering
%   \begin{subfigure}{0.49\textwidth}
%   \includegraphics[width=\linewidth]{Graphics/single_big.pdf}
%     \caption{Performance–efficiency trade-off of Qwen3-VL models.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.49\textwidth}
%   \includegraphics[width=\linewidth]{Thinking-Instruct-Compare.pdf}
%     \caption{Impact of max new token length on model performance across Qwen3-VL models.}
%     \label{fig:max_new_token_length}
%   \end{subfigure}
%   \caption{Efficiency exploration of Qwen3-VL model family.}
%   \label{fig:short}
% \end{figure}


% \begin{tabularx}{\columnwidth}{|X|X|X|} % X 代表自动伸缩的列


% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{l c c c}
% \toprule
% \textbf{Model} & \textbf{Count} & \textbf{Bbox} & \textbf{C.Score} \\
% \midrule

% Claude-Sonnet-4-6-Think 
% & \checkmark & \checkmark & 70.49 \\
% & \checkmark &  & 66.98 {\color{blue}(-3.51)} \\
% \midrule

% Qwen3-VL-235B-A22B-Think
% & \checkmark & \checkmark & 72.80 \\
% & \checkmark &  & 70.29 {\color{blue}(-2.51)} \\
% \midrule

% Qwen3.5-122B-A10B
% & \checkmark & \checkmark & 67.12 \\
% & \checkmark &  & 67.03 {\color{blue}(-0.09)} \\
% \midrule

% Qwen3-VL-235B-A22B-Ins
% & \checkmark & \checkmark & 66.20 \\
% & \checkmark &  & 62.38 {\color{blue}(-3.82)} \\
% \midrule

% InternVL3.5-241B-A28B
% & \checkmark & \checkmark & 61.87 \\
% & \checkmark &  & 64.32 {\color{red}(+2.45)} \\
% \bottomrule

% \end{tabular}
% \caption{Counting Score comparison between joint localization-and-count setting and count-only setting. ``C.Score'' denotes the Counting Score.}
% \label{tab:fig_5.2.2}
% \end{table}


\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt} % 调整列间距，默认是6pt
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}X c c c}
\toprule
\textbf{Model} & \textbf{Count} & \textbf{Bbox} & \textbf{C.Score} \\
\midrule

\multirow{2}{*}{Claude-Sonnet-4-6$^{\dagger}$}
& \checkmark & \checkmark & 70.49 \\
& \checkmark &  & 66.98 {\color{blue}(-3.51)} \\
\midrule

\multirow{2}{*}{Qwen3-VL-235B-A22B$^{\dagger}$}
& \checkmark & \checkmark & 72.80 \\
& \checkmark &  & 70.29 {\color{blue}(-2.51)} \\
\midrule

\multirow{2}{*}{Qwen3.5-122B-A10B}
& \checkmark & \checkmark & 67.12 \\
& \checkmark &  & 67.03 {\color{blue}(-0.09)} \\
\midrule

\multirow{2}{*}{Qwen3-VL-235B-A22B}
& \checkmark & \checkmark & 66.20 \\
& \checkmark &  & 62.38 {\color{blue}(-3.82)} \\
\midrule

\multirow{2}{*}{InternVL3.5-241B-A28B}
& \checkmark & \checkmark & 61.87 \\
& \checkmark &  & 64.32 {\color{red}(+2.45)} \\
\bottomrule
\end{tabularx}
\caption{Counting Score comparison between joint localization-and-count setting and count-only setting. ``C.Score'' denotes the Counting Score. $^{\dagger}$ denotes models evaluated with thinking mode.}
\label{tab:fig_5.2.2}
\end{table}






\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt} 
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}X l c}
\toprule
\textbf{Model} & \textbf{Overlay Type} & \textbf{Score} \\
\midrule

\multirow{3}{*}{Claude-Sonnet-4-6$^{\dagger}$}
& w/o Overlay & 33.95 \\
& Bbox & 36.77 {\color{red}(+2.82)} \\
& Mask & 45.38 {\color{red}(+11.43)} \\
\midrule

\multirow{3}{*}{Qwen3-VL-235B-A22B$^{\dagger}$}
& w/o Overlay & 35.56 \\
& Bbox & 37.60 {\color{red}(+2.04)} \\
& Mask & 41.73 {\color{red}(+6.17)} \\
\midrule

\multirow{3}{*}{Qwen3.5-122B-A10B}
& w/o Overlay & 31.61 \\
& Bbox & 32.79 {\color{red}(+1.18)} \\
& Mask & 32.28 {\color{red}(+0.67)} \\
\midrule

\multirow{3}{*}{Qwen3-VL-235B-A22B}
& w/o Overlay & 28.90 \\
& Bbox & 32.85 {\color{red}(+3.95)} \\
& Mask & 32.70 {\color{red}(+3.80)} \\
\midrule

\multirow{3}{*}{InternVL3.5-241B-A28B}
& w/o Overlay & 41.18 \\
& Bbox & 43.97 {\color{red}(+2.79)} \\
& Mask & 43.12 {\color{red}(+1.94)} \\
\bottomrule

\end{tabularx}
\caption{Performance comparison between Thinking and Instruct models under different overlay types, with $^{\dagger}$ denoting models evaluated with thinking mode.}
\label{tab:overlay_bbox_mask_comparison}
\end{table}


% \begin{table}[t]                                               
% \centering    
% \caption{Comparison of different models on the TL+CR benchmark.}               
% \label{tab:model_comparison} 
% \begin{tabular}{lccc}
%   \toprule
%   \multirow{2}{*}{Model}
%     & Full          & Full                & Ablation \\
%     & mean(score)   & mean(count score)  & mean(count score)\\
%   \midrule
%   Claude-Sonnet-4-6-Thinking  & 43.57 & 70.49 & 66.98 \\
%   Qwen3-VL-235B-A22B-Thinking    & \textbf{55.06} & \textbf{72.80} & \textbf{70.29} \\
%   Qwen3.5-122B-A10B              & 48.12 & 67.12 & 67.03 \\
%   Qwen3-VL-235B-A22B-Instruct    & 46.32 & 66.20 & 62.38 \\
%   InternVL3.5-241B-A28B          & 46.07 & 61.87 & 64.32 \\
%   \bottomrule
% \end{tabular}
% \end{table}



\subsection{Model Efficiency Assessment}
\label{sec:model_efficiency}
% we investigate the effect of output length on 
% model performance, with the aim of providing practical guidance for selecting VLMs in downstream embodied agent deployment.

% Figure~\ref{fig:max_new_token_length} compares final scores of models under different max-new-tokens settings.

% \textbf{4096 Output Length} When the maximum output length is constrained to 4,096 tokens, we observe that small- and medium-sized thinking models exhibit a high frequency of truncated responses, whereas non-thinking models of comparable scale encounter this issue far less often, as do larger thinking models. Under this setting, small- and medium-sized thinking models score below their non-thinking counterparts of equivalent scale. This suggests that, when faced with challenging problems, larger thinking models reason more efficiently within a constrained token budget.


% \textbf{8192 Output Length}When the maximum output length is relaxed to 8,192 tokens or beyond, truncation becomes substantially less frequent, and the overall scores of thinking models improve across the board. Notably, medium-sized models exhibit a larger score gain than both large and small models. Furthermore, medium-sized thinking models come to outperform their non-thinking counterparts under this setting. This indicates that, for challenging tasks, inference-time scaling is particularly effective for small- and medium-sized models.

% Real-world deployment scenarios require a joint consideration of efficiency and effectiveness. As shown in Figure~\ref{fig_5.4.2}, we plot a performance-efficiency figure, in which models positioned closer to the upper-right corner exhibit a more favorable performance-efficiency trade-off.
We analyze the inference efficiency of the Qwen3-VL family, focusing on generation length constraints and performance-efficiency trade-off.

\paragraph{Impact of Generation Length Constraints.} The parameter \textit{max new token} disproportionately limits Thinking models, which require extended budgets to formulate complete reasoning chains. Under a constrained budget (4096 tokens), small-scale Thinking models frequently suffer from response truncation, underperforming their standard Instruct counterparts (Fig.~\ref{fig:short-a}). Conversely, extending the limit to 8,192 tokens yields consistent gains, allowing large-scale Thinking models to fully leverage their reasoning capabilities and achieve optimal results.

\paragraph{Performance-Efficiency Trade-off.} As shown in Fig.~\ref{fig:short-b}, Thinking variants generally improve performance when sufficient generation budget is available, but their gains are accompanied by substantially higher latency and are sensitive to token truncation. In resource-constrained or latency-sensitive scenarios, small-scale Instruct models remain the more practical choice. Consequently, to prevent premature truncation of reasoning chains, we strongly recommend allocating a minimum generation budget of 8,192 tokens when deploying Thinking variants.




==> sections/intro.tex <==
\section{Introduction}
Vision is the primary modality through which embodied agents perceive the physical world, forming the foundation for downstream reasoning and planning. With the rapid advancement of large vision–language models (VLMs), these models have increasingly been adopted as the perceptual backbone of embodied systems~\cite{zhang2025embodied, Pelican-VL,ERQA,RoboBrain2.5,GR-1.5}, and corresponding benchmarks have been proposed to evaluate their capabilities in perception, reasoning, and planning~\cite{ERQA,EmbSpatial-Bench,RoboSpatial,RoboAfford++,EmbodiedBench,RynnBrain}. Nevertheless, a fundamental question remains: \textbf{Can current VLMs generalize to real-world embodied visual perception tasks?} Answering this question requires systematic benchmarking to understand the extent to which existing VLMs can support embodied deployment and to identify the perceptual capabilities that still require improvement.

Embodied visual perception requires not only recognizing the existence of a target object but also precisely determining its spatial location to support downstream tasks such as navigation and manipulation. However, traditional visual benchmarks commonly rely on question-answering (QA)~\cite{OpenEQA,EmbodiedBench,EXPRESS-Bench} or multiple-choice (MCQ) formats~\cite{EmbSpatial-Bench,ERQA,OmniSpatial}. Such protocols may yield overly optimistic evaluations of embodied perception, as models can exploit linguistic priors and common-sense reasoning instead of demonstrating genuine visual grounding ability. The detailed comparison is represented in Tab.~\ref{tab:benchmark_comparison}.

Within embodied visual perception, visual grounding, the process of localizing language instructions with specific objects and spatial locations in the physical environment, is a fundamental capability. However, existing visual grounding benchmarks only partially capture this requirement by predominantly focusing on object detection in generic scenes \cite{RefCOCO-test,DOD,OmniLabel}. Many tasks reduce to category-level retrieval with relatively simple textual descriptions or lack task-oriented perception requirements that are critical in embodied environments \cite{GRES,RefCOCO-test}.

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{Graphics/Overall/final_teaser.pdf}
%   \caption{Overview of EPIC-Benchmark.}
%   \label{fig:teaser}
% \end{figure*}



Although recent embodied perception benchmarks have begun to examine specific capabilities, such as spatial relation understanding and free-space detection~\cite{OmniSpatial,RoboSpatial,EmbSpatial-Bench}, a comprehensive and systematic evaluation of embodied visual perception remains lacking. To bridge this gap, we introduce \textbf{EPIC-Bench}, a comprehensive benchmark for embodied visual perception comprising 6,661 testing instances organized into 9 subcategories and 23 tasks. It covers the fine-grained perception pipeline required for embodied agents: from localizing the target object upon receiving an instruction, to reasoning about navigation toward it, and ultimately supporting task-specific manipulation. We adopt mask grounding as the primary evaluation protocol, complemented by three additional scoring metrics to provide multi-dimensional assessment.
% The benchmark is organized into 9 subcategories and 23 tasks, allowing a fine-grained diagnosis of perception deficiencies in current VLMs in embodied settings.
% Our work highlights the necessity of rethinking the evaluation of VLMs from an embodied perspective and provides a practical foundation for future progress.
The key contributions of our paper can be summarized below:
\begin{itemize}

\item We introduce \textbf{EPIC-Bench}, a large-scale benchmark specifically designed to evaluate mask-level embodied visual perception in VLMs. It comprises 6,661 testing instances across 9 subcategories and 23 tasks. To ensure annotation quality, we employ 20 human annotators with undergraduate-level education, accumulating over 4,800 person-hours of annotation effort across 30 working days. The benchmark is publicly available.

\item \textbf{The evaluation framework centered on mask grounding} mitigates shortcut exploitation from language priors and better reflects perception requirements in embodied environments.

\item We conduct \textbf{extensive experiments and ablation studies} on a diverse set of 89 representative VLMs. Our findings provide actionable insights into current limitations and offer guidance for future research on embodied downstream improvement.
\end{itemize}


==> sections/related_work.tex <==
\section{Related Work}

% In this section, we review the related work around two topics: \textit{embodied} and \textit{visual grounding} benchmarks, to highlight the current research limitation and elucidate the motivation underlying our work. A summarization of embodied visual perception and grounding based benchmarks are provided in \Cref{tab:benchmark_comparison}.

\paragraph{Vision Language Models for Embodied Tasks.}
A growing body of work leverages VLMs to build embodied systems. \textit{Gemini Robotics-ER}\cite{Gemini_Robotic,Gemini_Robotic_1.5} extends Gemini's multimodal reasoning capabilities into the physical world. Many recent studies have worked on language-guide task like navigation and manipulation, \textit{LERF}~\cite{kerr2023lerf} queries conditions on object masking to separate sub-parts of the object. \textit{ShapeGrasp}~\cite{li2024shapegrasp} infers contact points by prompting the VLMs via Chain of Thought.

% \textcolor{blue}{[reviewers' mentioned ref]}

% BLINK: Multimodal Language Models Can See but Not Perceive

% RoboRefer: Towards Spatial Referring with Reasoning in Vision-Language Models for Robotics

% RoboSpatial: Teaching Spatial Understanding to 2D and 3D Vision-Language Models for Robotics

% BEAR: Benchmarking and Enhancing Multimodal Language Models for Atomic Embodied Capabilities

% Robobench: A Comprehensive Evaluation Benchmark for Multimodal Large Language Models as Embodied Brain

% NaviTrace

% “ScanRefer: 3D Object Localization in RGB-D Scans using Natural Language” [Chen et al. 2020]

% “ReferIt3D: Neural Listeners for Fine-Grained 3D Object Identification in Real-World Scenes” [Achlioptas et al. 2022]

% “Text2Loc: 3D Point Cloud Localization from Natural Language” [Xia et al. 2024]

% “ViGiL3D: A Linguistically Diverse Dataset for 3D Visual Grounding” [Wang et al. 2025]

% \subsection{Visual Grounding}
\paragraph{Visual Grounding.}
Visual grounding requires models to localize target objects based on textual descriptions. \textit{RefCOCO-test}~\cite{RefCOCO-test} is among the most representative benchmarks, though its annotations assume exactly one target per description. \textit{$D^3$}~\cite{DOD} and \textit{OmniLabel}~\cite{OmniLabel} extend to complex language-based detection but adopt bounding-box annotations, which are less suitable for embodied scenarios requiring fine-grained localization of irregular objects. \textit{GRES}~\cite{GRES} introduces mask-level annotations; however, it focuses on generic scene understanding rather than embodied perception tasks.
% Visual grounding is a classic task for evaluating visual perception capability, where a model is required to localize a target object in an image based on a textual description. Among existing benchmarks, \textit{RefCOCO-test}~\cite{RefCOCO-test} is one of the most representative benchmarks, with annotations typically assuming that exactly one object in the image corresponds to the provided description. Beyond this setting, \textit{$D^3$}~\cite{DOD} and \textit{OmniLabel}~\cite{OmniLabel} focus on complex language-based object detection tasks, where ground-truth annotations are provided in bounding-box (Bbox) format. However, such box-level representation is less suitable for embodied scenarios, which often require more fine-grained localization or involve objects with irregular shapes. To address this limitation, \textit{GRES}~\cite{GRES} introduces mask-level annotations for grounding. Nevertheless, it is primarily designed for generic scene understanding. As a result, its labeling taxonomy and task organization do not explicitly follow a perception framework oriented toward embodied environments.

% \subsection{Embodied Benchmarks}
\paragraph{Embodied Benchmarks.}
Several benchmarks have been proposed to evaluate visual perception capabilities in embodied scenarios. \textit{EmbSpatial}~\cite{EmbSpatial-Bench} constructs template-based MCQs to assess model’s understanding of six canonical spatial relations. \textit{RoboSpatial-Home}~\cite{RoboSpatial} and \textit{RefSpatial-Bench}~\cite{RoboRefer} adopts point selection and binary-choice formats to evaluate spatial relation reasoning and object placement understanding.\textit{OpenEQA}~\cite{OpenEQA} and \textit{ERQA}~\cite{ERQA} evaluate multimodal understanding abilities associated with target localization and manipulation-oriented reasoning. \textit{RoboAfford-Eval}~\cite{RoboAfford++} focuses on localization capabilities relevant to grasping operations, along with global target localization and free-space identification. 

% Overall, these benchmarks predominantly adopt QA, MCQ, or point-based evaluation formats. Moreover, they typically assess only a subset of the capabilities required to complete a full embodied instruction pipeline. Consequently, they fall short of providing a comprehensive evaluation of embodied visual perception: an important gap that our work aims to address.

Overall, these benchmarks predominantly adopt QA, MCQ, or point-based evaluation formats. Moreover, they typically assess only a subset of the capabilities required to complete a full embodied instruction pipeline. Consequently, they fall short of providing a comprehensive evaluation of embodied visual perception: an important gap that our work aims to address. A detailed comparison of existing benchmarks is provided in Tab.~\ref{tab:benchmark_comparison}.

% Building upon these prior efforts, our work further advances visual grounding evaluation by explicitly focusing on embodied visual perception. In the next section, we will introduce our EPIC-Bench, enabling a more comprehensive and practically relevant assessment of perception capabilities in embodied scenarios.


\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
% \resizebox{\textwidth}{!}{
\begin{tabular}{l l |ccc ccc ccc| c |c| c l}
\toprule
\multirow{2}{*}{\textbf{Benchmark / Dataset}} &
\multirow{2}{*}{\textbf{GT Type}} &
\multicolumn{3}{c}{\textbf{Target Localization}} &
\multicolumn{3}{c}{\textbf{Navigation}} &
\multicolumn{3}{c|}{\textbf{Manipulation}} &
\multirow{2}{*}{\textbf{Data Domain}} &
\multirow{2}{*}{\textbf{Manual}} &
\multirow{2}{*}{\textbf{\makecell{Multi\\View}}} &
\multirow{2}{*}{\textbf{Size}} \\

\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
& & \textbf{BA} & \textbf{SRA} & \textbf{ECA} & \textbf{GD} & \textbf{FP} & \textbf{VM} & \textbf{AR} & \textbf{CR} & \textbf{PR} & & & & \\
\midrule

EmbSpatial-Bench\cite{EmbSpatial-Bench} & MCQ & \cmark & \cmark &   &   &   &   &   &   &   & Ind. &  &  & 3.6k \\
RoboSpatial-Home\cite{RoboSpatial} & Point+Binary & \cmark & \cmark &   &   &   &   &   &   & \cmark & Ind. & \cmark &  & 350 \\
RefSpatial-Bench\cite{RoboRefer} & Point/Mask & \cmark & \cmark &   &   &   &   &   &   & \cmark & Gen./Ind. & \cmark &  & 200 \\
OmniSpatial\cite{OmniSpatial} & MCQ & \cmark & \cmark & \ding{51}$^{\dagger}$ &   &   &   & \cmark &   &   & Gen./Ind. & \cmark &  & 8.4k \\

OpenEQA \cite{OpenEQA}& QA & \cmark & \cmark & \cmark &   &   &   & \cmark &   &   & Ind./Ego. & \cmark & \cmark & 1.6k \\
ERQA\cite{ERQA} & MCQ & \cmark & \cmark & \cmark &   &   & \cmark & \cmark & \cmark & \cmark & Ind./Ego./Robo & \cmark & \cmark & 400 \\

RoboAfford-Eval\cite{RoboAfford++} & Point & \cmark & \ding{51}$^{\dagger}$ &   & \ding{51}$^{\dagger}$ &   &   & \cmark &   & \cmark & Gen./Ind./Robo./Ego. & \cmark &  & 338 \\
EmbodiedBench\cite{EmbodiedBench} & QA & \cmark & \ding{51}$^{\dagger}$ & \ding{51}$^{\ddagger}$ &   & \cmark &   & \cmark &   & \cmark & Ind./Robo. & \ding{51}$^{\ddagger}$ & \cmark & 1.1k \\
EXPRESS-Bench\cite{EXPRESS-Bench}& QA & \cmark & \cmark & \cmark &   &   &   &   &   &   & Ind. & \cmark &  & 2.0k \\
RynnBrainBench\cite{RynnBrain}& QA+Point & \cmark & \cmark & \cmark &   &   &   & \cmark &   & \cmark & Ind./Robo./Ego. &  & \cmark & 12k \\

\midrule

RefCOCO-test\cite{RefCOCO-test} & BBox & \cmark & \cmark &   &   &   &   &   &   &   & Gen. & \ding{51}$^{\ddagger}$ &  & 10.7k \\
DOD \cite{DOD} & BBox & \cmark & \cmark & \ding{51}$^{\dagger}$ &   &   &   &   &   &   & Gen. & \ding{51}$^{\ddagger}$ &  & 24.2k \\
OmniLabel \cite{OmniLabel} & BBox & \cmark & \cmark & \ding{51}$^{\dagger}$ &   &   &   &   &   &   & Gen. &  \ding{51}$^{\ddagger}$&  & 15.8K \\
GRES\cite{GRES} & Mask & \cmark & \cmark & \ding{51}$^{\dagger}$ &   &   &   &   &   &   & Gen. &  &  & 60.2k \\

\midrule
\rowcolor{blue!8}
\textbf{EPIC-Bench} & \textbf{Mask+Count} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{Gen./Ind./Robo./Ego.} &\textbf{\cmark} &\textbf{\cmark} & \textbf{6.6k} \\

\bottomrule
\end{tabular}
% }
\caption{Comparison of perception benchmarks/datasets.  $^{\dagger}$ denotes partial support;  $^{\ddagger}$ denotes the dataset is auto-generated with manual selection.}
\label{tab:benchmark_comparison}
\end{table*}









% \label{sec:intro}
% Recent works focus on building embodied system upon powerful generic pretrained LVLMs\cite{team2025gemini,GR-1.5}, which have demonstrated remarkable capabilities in perception, understanding and planning when tackling complex problems across domains. However, can state-of-the-art VLMs trained on generic multimodal dataset perform effectively in real world embodied perception tasks? What specific limitations remain, and which capabilities require further improvement? Existing generic VLM benchmarks are not designed to answer these questions. To address this gap, we introduce an embodied perception grounding benchmark.

% We focus on visual perception, as it serves as the foundation for downstream understanding and planning. Vision is the most fundamental and direct channel through which an embodied agent acquires information from the physical world, making robust visual grounding a prerequisite for reliable embodied intelligence.





% In recent years, Large Multimodal Models (LMMs) have increasingly been adopted as the cognitive backbone of embodied agents, or further extended into Vision-Language-Action (VLA) models to inherit their strong general-purpose perception, understanding, and planning capabilities learned from large-scale web data (e.g., \cite{GR-1.5}).

% Despite the emerging trend of leveraging VLMs for embodied control, a fundamental question remains underexplored: do the perceptual capabilities learned from generic internet-scale training sufficiently support the fine-grained requirements of real-world embodied tasks? Human daily activities often demand precise object localization, spatial reasoning, interaction understanding, and affordance perception—abilities that are not explicitly optimized in standard VLM training objectives.

% In this work, we focus on visual perception, as it serves as the foundation for downstream understanding and planning. For embodied agents, visual perception constitutes the most direct and primary channel for acquiring information from the physical world, and its quality fundamentally constrains the agent’s decision-making capacity.



% Embodied intelligence requires agents to perceive, reason, and act within physical environments. Unlike purely textual reasoning systems, embodied agents must ground language instructions into fine-grained perceptual representations that support localization, navigation, and manipulation. This grounding process demands more than coarse spatial awareness; it requires precise object identification, relational understanding, and region-level reasoning.

% Recent multimodal large models (VLMs) have demonstrated impressive performance on a variety of benchmarks. However, closer inspection reveals a critical limitation: most existing benchmarks emphasize high-level spatial reasoning, visual question answering, or multiple-choice formats. These evaluation protocols often prioritize semantic plausibility over precise perceptual grounding. As a consequence, they insufficiently capture the perceptual granularity required in embodied scenarios.

% Specifically, three gaps remain:

% \textbf{Insufficient fine-grained perception evaluation.}
% Many benchmarks focus on global reasoning or image-level understanding, while embodied tasks demand region-level, instance-level, and mask-level precision.

% \textbf{Limited embodied task coverage.}
% Existing VLM benchmarks emphasize spatial reasoning but rarely evaluate dimensions directly related to embodied execution, such as object localization for manipulation, navigation-oriented grounding, or multi-step interaction cues.

% \textbf{Evaluation format limitations.}
% Multiple-choice (MCQ) and question-answering (QA) paradigms allow models to exploit language priors or probabilistic guessing strategies. These formats may obscure failures in precise perception. In contrast, region-level or mask-level evaluation provides a more faithful measurement of perceptual competence, avoiding shortcut solutions.

% To address these challenges, we propose EPIC-Bench, a comprehensive fine-grained grounding benchmark tailored for embodied perception evaluation. Unlike prior benchmarks, EPIC-Bench explicitly measures localization accuracy, relational grounding precision, and manipulation-relevant perceptual capability. By incorporating high-quality mask-level annotations, the benchmark provides a more rigorous and spatially precise evaluation protocol.

% % We further introduce EPIC-Bench-Lite, a compact yet representative subset designed for rapid benchmarking and ablation studies. Together, these two benchmarks establish a systematic evaluation framework for multimodal models in embodied contexts.

% Extensive experiments across a broad set of mainstream multimodal large models demonstrate a consistent gap between current model capabilities and embodied perceptual requirements. Even the strongest frontier systems show significant weaknesses in fine-grained grounding scenarios. Through comprehensive data and performance analysis, we show that EPIC-Bench reveals limitations previously hidden by coarse evaluation protocols.

% Our work highlights the necessity of rethinking multimodal evaluation from an embodied perspective and provides a practical foundation for future progress.The key contributions of our paper can be summarized below:
% \begin{itemize}
%     \item \textbf{EPIC-Bench}: We introduce EPIC-Bench, a large-scale fine-grained embodied grounding benchmark designed to evaluate multimodal models from an embodied perception perspective. The benchmarks span 3 main categories, 9 types of tasks and 21 subcategories, covering localization, navigation-relevant grounding, and manipulation-oriented perception.
%     \item \textbf{Bias-Resistant Evaluation Design}: We move beyond traditional MCQ and QA formats by incorporating fine-grained and mask-level spatial annotations, enabling more faithful evaluation of perceptual precision and reducing shortcut exploitation through language priors.
%     \item \textbf{Experimental Results}: We systematically evaluated a broad spectrum of state-of-the-art multimodal large models across different architectures and scales. Our findings reveal that even the most advanced frontier models exhibit substantial limitations in fine-grained perceptual grounding.
%     \item \textbf{Data and Experiment Analysis}: We provide detailed statistical analysis of data diversity, annotation quality, and task difficulty. Our experimental insights highlight the gap between current multimodal reasoning benchmarks and embodied perceptual requirements, with the hope of providing valuable experience for the community's future development.
% \end{itemize}


% \begin{figure*}[th]
%     \centering
%     \includegraphics[width=1\textwidth]{bmk_cases.png}
%     \caption{Examples of EPIC-Bench.}
%     \label{fig:data_sample}
% \end{figure*}









==> tabs/main_eval_results_bak.tex <==


%\cellcolor{green!10}。\underline
\begin{table*}[htb]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    % \fontsize{5}{5}\selectfont
    \renewcommand{\arraystretch}{1} % 统一行距
    % \resizebox{\textwidth}{!}{%
    % \small
    \footnotesize
    \begin{tabular}{l c ccc ccc ccc}    \toprule
    \multirow{3}{*}{\textbf{Model}}
        & \multirow{3}{*}{\textbf{Average}}
        & \multicolumn{3}{c}{\textbf{Target Local.}}
        & \multicolumn{3}{c}{\textbf{Navigation}}
        & \multicolumn{3}{c}{\textbf{Manipulation}} \\
    \cmidrule(r){3-5} \cmidrule(r){6-8} \cmidrule(r){9-11}
    &  & BA & SRA & ECA & GD & FP & VM & AR & CR & PR. \\
    \midrule

    \rowcolor{blue!8}[0pt][0pt]
    \multicolumn{11}{@{}c@{}}{\textbf{Proprietary Models}} \\
  
    % Gemini-2.5-Pro$^{\dagger}$           & 37.63 & 42.86 & 41.62 & 36.43 & 9.630  & 46.29 & 42.70 & 8.720 & 33.94 & 42.78 \\
    Gemini-3-Pro$^{\dagger}$ &\colorbox{green!10}{\textbf{54.81}}& \underline{56.81} & \underline{54.50} & \colorbox{green!10}{\textbf{53.90} }& \underline{48.82} & \colorbox{green!10}{\textbf{70.82} }& \colorbox{green!10}{\textbf{60.08}}
    & \colorbox{green!10}{\textbf{30.40}} & \colorbox{green!10}{\textbf{51.78}} & \colorbox{green!10}{\textbf{53.42} }\\
    % Gemini-3.1-Pro$^{\dagger}$           & \underline{54.72} & 55.38 & \cellcolor{green!10}\textbf{56.65} & \underline{53.04} & 47.22 & \underline{70.32} & \uquadnderline{59.06} & \underline{28.89} & \cellcolor{green!10}\textbf{53.70} & \cellcolor{green!10}\textbf{55.25} \\
    
    Claude-Sonnet-4.6$^{\dagger}$         & 43.24 & 45.43 & 45.49 & 36.47 & 40.16 & \underline{68.46} & 42.77 & 9.790 & 46.21 & 43.81 \\
    
    % o3$^{\dagger}$    & 36.05 & 39.37 & 40.96 & 32.86 & 36.24 & 30.64 & 40.73 & 5.49 & 32.43 & 43.64 \\
    % GPT-5.4                                      & 38.95 & 43.78	&43.90	&33.84	&32.24	&43.12	&44.35	&8.670	&39.55	&37.30 \\
   
    GPT-5.5                       & 50.16 & \textbf{57.78}	&\textbf{55.37}	&45.19	&\textbf{50.97}	&38.57	& \underline{51.65}	& \underline{24.62}	& \underline{49.67}	& \underline{48.70} \\
    
    Doubao-Seed-1.8$^{\dagger}$           & \underline{46.32} & 55.29 & 49.68  & \underline{46.10} & 46.02 & 53.43 & 45.90 & 10.94 & 14.36 & 40.79 \\
    % Doubao-Seed-1.6-Vision$^{\dagger}$    & 46.80 & 54.64 & 49.92  & 42.27 & 41.64 & 58.74 & 42.66 & 9.520 & 47.48 & 41.62 \\

    Qwen3.6-Plus$^{\dagger}$              & 45.48 & 47.66 & 50.17  & 41.07 & 44.47 & 62.12 & 41.57 & 11.95 & 47.84 & 41.59 \\
    % Qwen3.5-Plus$^{\dagger}$              & 47.10 & 55.09 & 51.90  & 41.82 & 50.85 & 57.89 & 45.21 & 13.82 & 22.34 & 42.46 \\
    % Qwen3.6-35B-A3B$^{\dagger}$           & 35.07 & 48.17 & 43.99  & 36.61 & 14.41 & 33.97 & 21.30 & 2.840 & 17.05 & 15.90 \\

    HunYuan-T1-Vision$^{\dagger}$         & 43.00 & 51.24 & 47.60  & 39.67 & 42.63 & 50.08 & 33.54 & 6.630  & 38.95 & 34.49 \\
    % HunYuan-Vision-1.5                    & 32.55 & 38.37 & 39.60 & 29.67 & 31.72 & 17.07 & 35.71  & 6.380  & 32.88 & 29.25 \\

    
    \midrule
    
    \rowcolor{blue!8}[0pt][0pt]
    \multicolumn{11}{@{}c@{}}{\textbf{Open-source Models}} \\
    % Qwen3.6-35B-A3B                     & 38.52 & 46.40 & 46.19 & 40.01 &  3.900 & 39.16 & 39.42 &  5.410 & 34.19 & 34.52 \\

    % Qwen3.5-397B-A17B$^{\dagger}$       & \underline{47.47} & \underline{55.45} & 51.82 & 42.10  & 51.10  & \underline{60.11} & \underline{45.35} & 12.40  & 26.33 & \underline{42.51} \\
    % Qwen3.5-397B-A17B                   & 45.16 & 50.56 & 50.06 & \underline{43.45} & \cellcolor{green!10}\textbf{51.94} & 50.61 & 41.46 & 8.310  & 34.51 & 37.08 \\
    % Qwen3.5-122B-A10B$^{\dagger}$       & 47.24 & 53.61 & 49.13 & 41.16 & \underline{51.42} & \textbf{63.47} & 45.19 & 12.31 & \underline{46.04} & 39.77 \\
    % Qwen3.5-122B-A10B                   & 44.54 & 50.77 & 49.28 & 42.31 & 49.65 & 50.50  & 42.62 & 8.300  & 36.91 & 32.16 \\

    Qwen3-VL-235B-A22B$^{\dagger}$      & \textbf{50.93} & \colorbox{green!10}{\textbf{58.00}} & \colorbox{green!10}{\textbf{55.67}}   & \textbf{48.12} & \textbf{48.18} & \textbf{51.19} & \textbf{49.01} & \textbf{16.96} & \textbf{48.04} & \textbf{46.49} \\
    % Qwen3-VL-235B-A22B  & 42.64 & 50.12 & 45.86 & 39.34 & 50.96 & 43.14 & 38.69 & 12.00 & 34.55 & 35.71 \\
    
    % Qwen2.5-VL-72B & 42.51 & 47.54 & 49.79 & 40.92 & 49.45 & 42.49 & 37.08 & 14.77 & 21.21 & 35.90 \\

    InternVL3.5-241B-A28B & 40.75 & 44.65 & \underline{50.59} & 37.61 & 35.94 & 35.47 & 33.73 & \underline{16.85} & \underline{36.41} & 37.60 \\
   
    % InternVL3.5-38B                               & 42.54 & 48.69 & \underline{52.60} & 39.95 & 43.21 & 35.01 & 28.07 & \textbf{17.22} & 34.05 & 35.83 \\
    % InternVL3.5-30B-A3B                           & 29.71 & 30.96 & 39.11 & 27.03 & 45.43 & 24.11 & 17.24 & 8.410  & 18.75 & 25.30 \\

    % InternVL3-78B                                 & 36.04 & 40.68 & 44.56 & 32.78 & 35.98 & 30.55 & 34.93 & 6.900  & 29.07 & 31.69 \\

    MiMo-VL-7B-RL-2508                            &34.65	&36.65&	42.31	&34.92	&18.31	&36.90	&\underline{37.45}	&6.510	&30.37&	32.86 \\
    Gemma-3-27B-IT                                & 27.17 & 26.93 & 33.66 & 26.68 & 11.62 & 32.17 & 26.33 & 1.650  & 31.26 & 32.18 \\
    GLM-4.6V$^{\dagger}$                & \underline{42.84} & \underline{50.19} & 47.71 & \underline{37.89} & \underline{42.46} & \underline{51.11} & 36.55 & 8.320  & 34.14 & \underline{39.79} \\
    Step3-VL-10B                                  & 32.40 & 42.22 & 40.10 & 31.88 & 17.96 & 24.03 & 17.77 & 5.940  & 27.22 & 27.56 \\
    LLaVA-NeXT-72B                                & 20.40 & 26.54 & 29.42 & 19.93 & 14.18 & 6.340  & 6.190  & 2.990  & 12.75 & 18.63 \\
        
    
    
    \midrule

    \rowcolor{blue!8}[0pt][0pt]
    \multicolumn{11}{@{}c@{}}{\textbf{Segmentation-capable Models}} \\
    GLaMM-7B  & 28.03 & 37.64 & 27.26 & 18.92 & \colorbox{green!10}{\textbf{84.23}} & \underline{37.88} & 0.01 & 1.27 & 3.40 & 17.67 \\

    
    UFO-8B    & \textbf{42.39} & \textbf{50.29} & \textbf{51.21} & \textbf{34.31} & \underline{78.51}  & \textbf{45.45} & \underline{3.52} & \textbf{8.00} & \textbf{35.97} & \underline{30.21} \\

    
    LISA++-7B & \underline{37.17} & \underline{37.96} & \underline{50.22} & \underline{28.94} & 76.34 & 23.56 & \textbf{26.51} & \underline{6.70} & \underline{26.73} & \textbf{31.37} \\

    
    \midrule

    \rowcolor{blue!8}[0pt][0pt]
    \multicolumn{11}{@{}c@{}}{\textbf{Embodied Foundation Models}} \\
    Pelican1.0-VL-72B                             & \underline{35.29} & \underline{44.08} & \underline{42.11} & \underline{34.79} & \textbf{44.91} & 0.000  & \textbf{38.13} & \textbf{7.320} & 22.68 & \underline{37.96} \\

    RoboBrain2-32B                                & \textbf{39.32} & \textbf{50.66} & \textbf{49.67} & \textbf{38.83} & \underline{38.85} & 0.610  & \underline{37.63} & 0.080 & \textbf{36.22} & \textbf{39.61} \\
    
    % RoboBrain2.5-8B-NV                            & 23.81 & 24.81 & 32.88 & 24.97 & 22.57 & 1.660  & 27.98 & 1.130 & 24.98 & 24.03 \\
    RoboBrain2.5-8B-MT                            & 29.83 & 31.20 & 37.41 & 26.76 & 33.52 & \textbf{30.89} & 27.84 & 2.650 & \underline{25.45} & 24.34 \\
    
    % RynnBrain-8B                                  & 22.34 & 28.31 & 33.28 & 24.81 & 7.980  & 5.950  & 15.04 & 0.130 & 13.84 & 11.26 \\
    % RynnBrain-CoP-8B                              & 16.83 & 12.48 & 21.78 & 16.08 & 21.51 & \underline{22.51} & 13.58 & 0.280 & 19.62 & 18.09 \\
    RynnBrain-Plan-8B                             & 23.59 & 23.53 & 32.53 & 26.08 & 2.120 & 19.57  & 21.41 & 0.110 & 18.79 & 31.02 \\
    
    VeBrain                                       & 29.27 &	33.63 &	35.98 & 27.69 & 29.56 &	\underline{20.04}  & 27.58 & 2.850&19.25 & 32.30 \\
    Cosmos-Reason1-7B                             & 23.25 & 29.74 & 26.64 & 19.67 & 24.68 & 3.030  & 25.44 & \underline{5.370} & 22.12 & 32.75 \\



    \bottomrule
    \end{tabular}
    % }
    \caption{
        Overall performance of representative VLMs on EPIC-Bench.
        \colorbox{green!10}{\textbf{Green bold}} indicates the overall best result across all models.
        \textbf{Bold} and \underline{underline} indicate the best and second-best results within each model category, respectively.
        $^{\dagger}$ denotes models evaluated with thinking mode enabled.
        % Comprehensive results for all evaluated models are provided in Tab.~\ref{tab:table-performance-full} of Appendix.~\ref{app:additional_results}.
    }
    \label{tab:table-performance-select}
\end{table*}

==> tabs/vlm_grasp_exp.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}

\caption{
Localization and grasp success rates under different settings.
Cond. denotes grasp success conditioned on successful localization.
}
\label{tab:grasp_results}

\begin{tabularx}{\columnwidth}{lcccccc}

\toprule

\multirow{2}{*}{ }
&
\multirow{2}{*}{Loc.}
&
\multicolumn{2}{c}{Grasp (bbox)}
&
\multicolumn{2}{c}{Grasp (mask)}
&
\multirow{2}{*}{GT} \\

\cmidrule(lr){3-4}
\cmidrule(lr){5-6}

&
&
Overall
&
Cond.
&
Overall
&
Cond.
&
\\

\midrule

Complex
&
45.5
&
40.0
&
63.0
&
44.0
&
95.0
&
90.0 \\

Simple
&
80.0
&
54.0
&
57.5
&
76.0
&
85.0
&
90.0 \\

\bottomrule

\end{tabularx}

\end{table}
